Point Cloud Sequence Encoding for Material-conditioned Graph Network Simulators

Graph Network Simulators (GNSs) have emerged as powerful surrogates for complex physics-based simulation, offering inherent differentiability and orders-of-magnitude speedups over traditional solvers. However, GNSs typically assume access to the underlying material parameters, such as stiffness or viscosity, severely limiting their utility in realistic experimental settings. While recent meta-learning approaches address the parameter dependency by inferring properties from mesh trajectories, reconstructing a mesh from an observed scene is challenging. In this work, we introduce Point Cloud Encoding for Accurate Context Handling (PEACH), a novel framework that applies in-context learning on point clouds to adapt a learned simulator to unseen physical properties during inference. Our approach relies on a novel spatio-temporal point cloud sequence encoder, as well as two forms of auxiliary supervision to help improve simulation fidelity. We demonstrate that PEACH is capable of accurate zero-shot sim-to-real transfer on a challenging, dynamic scene. Experiments on simulation scenes show that PEACH even outperforms mesh-based baselines on prediction accuracy, while being much more practical for real-world deployment.

==> content/04_a_preliminaries.tex <==
\section{Preliminaries}
\begin{itemize}
    \item GNS/Mango
    \item Punktwolken
\end{itemize}

==> figures/quantitative_results/bbv/mat_prop_loss/bar_bbv_bar.tex <==
% This file was created with matplot2tikz v0.5.1.
\begin{tikzpicture}

\definecolor{darkgray}{RGB}{169,169,169}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{darkturquoise23190207}{RGB}{23,190,207}
\definecolor{gray127}{RGB}{127,127,127}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{orchid227119194}{RGB}{227,119,194}
\definecolor{sienna1408675}{RGB}{140,86,75}
\definecolor{steelblue31119180}{RGB}{31,119,180}
\definecolor{steelblue76114176}{RGB}{76,114,176}

\begin{axis}[
axis line style={darkgray},
log basis y={10},
tick align=outside,
title={Bending Beam},
x grid style={lightgray204},
xmajorgrids,
xmajorticks=false,
xmin=-0.63, xmax=6.63,
xtick style={color=darkslategray38},
xtick={0,1,2,3,4,5,6},
xticklabel style={rotate=45.0,anchor=east},
xticklabels={
  PEACH Encoder (ours),
  Mesh-based Encoder,
  No Context Encoding,
  MGN,
  MGN Oracle,
  GNN Encoder,
  PSTNet Encoder
},
y grid style={lightgray204},
ylabel=\textcolor{darkslategray38}{Material Properties MSE},
ymajorgrids,
ymin=0.0001, ymax=0.01,
ymode=log,
ytick pos=left,
ytick style={color=darkgray}
]
\draw[draw=white,fill=steelblue31119180] (axis cs:-0.3,0) rectangle (axis cs:0.3,0.201905166900158);
\draw[draw=white,fill=darkturquoise23190207] (axis cs:0.7,0) rectangle (axis cs:1.3,0.261850817298889);
\draw[draw=white,fill=gray127] (axis cs:1.7,0) rectangle (axis cs:2.3,0);
\draw[draw=white,fill=darkorange25512714] (axis cs:2.7,0) rectangle (axis cs:3.3,2.62958733568192);
\draw[draw=white,fill=mediumpurple148103189] (axis cs:3.7,0) rectangle (axis cs:4.3,2.62958733568192);
\draw[draw=white,fill=sienna1408675] (axis cs:4.7,0) rectangle (axis cs:5.3,0.824786586856842);
\draw[draw=white,fill=orchid227119194] (axis cs:5.7,0) rectangle (axis cs:6.3,2.74944473633766);
\draw [draw=black, semithick] (axis cs:0,0.183820147067308) -- (axis cs:0,0.218326382339001);
\draw [draw=black, semithick] (axis cs:-0.25,0.183820147067308) -- (axis cs:0.25,0.183820147067308);
\draw [draw=black, semithick] (axis cs:-0.25,0.218326382339001) -- (axis cs:0.25,0.218326382339001);

\draw [draw=black, semithick] (axis cs:1,0.225880924612284) -- (axis cs:1,0.323451224714518);
\draw [draw=black, semithick] (axis cs:0.75,0.225880924612284) -- (axis cs:1.25,0.225880924612284);
\draw [draw=black, semithick] (axis cs:0.75,0.323451224714518) -- (axis cs:1.25,0.323451224714518);

\draw [draw=black, semithick] (axis cs:2,0) -- (axis cs:2,0);
\draw [draw=black, semithick] (axis cs:1.75,0) -- (axis cs:2.25,0);
\draw [draw=black, semithick] (axis cs:1.75,0) -- (axis cs:2.25,0);

\draw [draw=black, semithick] (axis cs:3,2.55671906471252) -- (axis cs:3,2.687067091465);
\draw [draw=black, semithick] (axis cs:2.75,2.55671906471252) -- (axis cs:3.25,2.55671906471252);
\draw [draw=black, semithick] (axis cs:2.75,2.687067091465) -- (axis cs:3.25,2.687067091465);

\draw [draw=black, semithick] (axis cs:4,2.55671906471252) -- (axis cs:4,2.687067091465);
\draw [draw=black, semithick] (axis cs:3.75,2.55671906471252) -- (axis cs:4.25,2.55671906471252);
\draw [draw=black, semithick] (axis cs:3.75,2.687067091465) -- (axis cs:4.25,2.687067091465);

\draw [draw=black, semithick] (axis cs:5,0.666586965322495) -- (axis cs:5,0.98278620839119);
\draw [draw=black, semithick] (axis cs:4.75,0.666586965322495) -- (axis cs:5.25,0.666586965322495);
\draw [draw=black, semithick] (axis cs:4.75,0.98278620839119) -- (axis cs:5.25,0.98278620839119);

\draw [draw=black, semithick] (axis cs:6,1.3828150331974) -- (axis cs:6,4.21560209989548);
\draw [draw=black, semithick] (axis cs:5.75,1.3828150331974) -- (axis cs:6.25,1.3828150331974);
\draw [draw=black, semithick] (axis cs:5.75,4.21560209989548) -- (axis cs:6.25,4.21560209989548);

\end{axis}

\end{tikzpicture}


==> figures/quantitative_results/db/ml_loss/db_ablation_context.tex <==
% This file was created with matplot2tikz v0.5.1.
% This file was created with matplot2tikz v0.5.1.
\begin{tikzpicture}
\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray}{RGB}{169,169,169}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
    line width=0.8pt, % Makes the axis outline thicker/darker
    axis line style={black}, % Use solid black for maximum contrast
    log basis y={10},
    % Combined minor and major ticks
    ytick={1e-06, 2e-06, 3e-06, 4e-06, 6e-06, 1e-05, 2e-05, 3e-05, 4e-05, 6e-05, 1e-04, 2e-04, 3e-04, 4e-04, 6e-04},
    yticklabels={
        \(1{\times}10^{-6}\), \(2{\times}10^{-6}\), \(3{\times}10^{-6}\), \(4{\times}10^{-6}\), \(6{\times}10^{-6}\),
        \(10^{-5}\), \(2{\times}10^{-5}\), \(3{\times}10^{-5}\), \(4{\times}10^{-5}\), \(6{\times}10^{-5}\),
        \(10^{-4}\), \(2{\times}10^{-4}\), \(3{\times}10^{-4}\), \(4{\times}10^{-4}\), \(6{\times}10^{-4}\)
    },
    tick align=outside,
    % title={Deforming Block},
    xlabel={Context Size},
    xlabel style={font=\LARGE, color=black},
    ylabel={Full Rollout MSE}, % Added ylabel back
    ylabel style={font=\LARGE, color=black}, % Matching the "Darker" style
    tick label style={font=\large, color=black}, % Matching the "Darker" style
    xmajorgrids,
    xtick={1,2,3,4,5,6,7,8},           % Specify tick positions
    xticklabels={1,2,3,4,5,6,7,8},     % Specify tick labels
    xmajorticks=true,                  % Ensure ticks are enabled
    xtick pos=bottom,
    xmin=0.65, xmax=8.35,
    xtick style={color=black, line width=0.8pt},
    y grid style={lightgray!70}, % Slightly darker grid for better visibility
    ymajorgrids,
    ymin=0.94208220010013e-06, ymax=3.09143132540889e-06,
    ymode=log,
    ytick pos=left,
    ytick style={color=black, line width=0.8pt}
]
\path [draw=darkorange25512714, fill=darkorange25512714, opacity=0.2]
(axis cs:1,2.95462405119906e-06)
--(axis cs:1,2.45336601238932e-06)
--(axis cs:2,2.20497292957589e-06)
--(axis cs:3,2.11740757549705e-06)
--(axis cs:4,2.03107032348271e-06)
--(axis cs:5,1.9985720882687e-06)
--(axis cs:6,1.94296484323786e-06)
--(axis cs:7,1.94556162114168e-06)
--(axis cs:8,1.95145361203686e-06)
--(axis cs:8,2.32996734439439e-06)
--(axis cs:8,2.32996734439439e-06)
--(axis cs:7,2.3596542746418e-06)
--(axis cs:6,2.36665329111929e-06)
--(axis cs:5,2.44106007585287e-06)
--(axis cs:4,2.39378744595342e-06)
--(axis cs:3,2.4429660925307e-06)
--(axis cs:2,2.56724428027155e-06)
--(axis cs:1,2.95462405119906e-06)
--cycle;
\path [draw=mediumpurple148103189, fill=mediumpurple148103189, opacity=0.2]
(axis cs:1,1.99352103891215e-06)
--(axis cs:1,1.66243012245104e-06)
--(axis cs:2,1.59966228352459e-06)
--(axis cs:3,1.47524616522787e-06)
--(axis cs:4,1.46801022538057e-06)
--(axis cs:5,1.44900729992514e-06)
--(axis cs:6,1.43809398878147e-06)
--(axis cs:7,1.41286835741994e-06)
--(axis cs:8,1.40251364655342e-06)
--(axis cs:8,1.79910261977057e-06)
--(axis cs:8,1.79910261977057e-06)
--(axis cs:7,1.80700888563479e-06)
--(axis cs:6,1.76912186589107e-06)
--(axis cs:5,1.82960323513726e-06)
--(axis cs:4,1.79694262669727e-06)
--(axis cs:3,1.8341795851029e-06)
--(axis cs:2,1.88873465845063e-06)
--(axis cs:1,1.99352103891215e-06)
--cycle;
\path [draw=crimson2143940, fill=crimson2143940, opacity=0.2]
(axis cs:1,2.02769706447725e-06)
--(axis cs:1,1.40788753810739e-06)
--(axis cs:2,1.35791756861181e-06)
--(axis cs:3,1.32207259184725e-06)
--(axis cs:4,1.2835851350701e-06)
--(axis cs:5,1.28860116888063e-06)
--(axis cs:6,1.27854914921954e-06)
--(axis cs:7,1.27543921735196e-06)
--(axis cs:8,1.27874079680623e-06)
--(axis cs:8,1.69665094063021e-06)
--(axis cs:8,1.69665094063021e-06)
--(axis cs:7,1.65599628800805e-06)
--(axis cs:6,1.69140358252662e-06)
--(axis cs:5,1.70982760820948e-06)
--(axis cs:4,1.73124954017112e-06)
--(axis cs:3,1.76100652993227e-06)
--(axis cs:2,1.85751306958082e-06)
--(axis cs:1,2.02769706447725e-06)
--cycle;
\path [draw=forestgreen4416044, fill=forestgreen4416044, opacity=0.2]
(axis cs:1,1.44048956940424e-06)
--(axis cs:1,1.1951971146118e-06)
--(axis cs:2,1.19520160524189e-06)
--(axis cs:3,1.19519444297111e-06)
--(axis cs:4,1.19517227403776e-06)
--(axis cs:5,1.19496376811412e-06)
--(axis cs:6,1.19520450425625e-06)
--(axis cs:7,1.19520740327062e-06)
--(axis cs:8,1.19519626196052e-06)
--(axis cs:8,1.4497597362606e-06)
--(axis cs:8,1.4497597362606e-06)
--(axis cs:7,1.44975774674094e-06)
--(axis cs:6,1.44050022754527e-06)
--(axis cs:5,1.44975012972282e-06)
--(axis cs:4,1.44973930105152e-06)
--(axis cs:3,1.44975649618573e-06)
--(axis cs:2,1.44974879390247e-06)
--(axis cs:1,1.44048956940424e-06)
--cycle;
\path [draw=steelblue31119180, fill=steelblue31119180, opacity=0.2]
(axis cs:1,1.81762419515508e-06)
--(axis cs:1,1.45395972594997e-06)
--(axis cs:2,1.38173538744013e-06)
--(axis cs:3,1.33824292376517e-06)
--(axis cs:4,1.33626258502773e-06)
--(axis cs:5,1.29966741724274e-06)
--(axis cs:6,1.31520494051074e-06)
--(axis cs:7,1.30778784068752e-06)
--(axis cs:8,1.31355028543112e-06)
--(axis cs:8,1.68259728638986e-06)
--(axis cs:8,1.68259728638986e-06)
--(axis cs:7,1.72052705238457e-06)
--(axis cs:6,1.68917330256591e-06)
--(axis cs:5,1.6862453549038e-06)
--(axis cs:4,1.70081307260261e-06)
--(axis cs:3,1.70971210877724e-06)
--(axis cs:2,1.73661598523722e-06)
--(axis cs:1,1.81762419515508e-06)
--cycle;
\addplot [very thick, darkorange25512714, mark=*, mark size=5, mark options={solid,draw=white}]
table {%
1 2.73071873380104e-06
2 2.39898594145416e-06
3 2.28819567382743e-06
4 2.2100099954514e-06
5 2.20702219166924e-06
6 2.15425234273425e-06
7 2.13807220461604e-06
8 2.1268699583743e-06
};
\addplot [very thick, mediumpurple148103189, mark=square*, mark size=5, mark options={solid,draw=white}]
table {%
1 1.87011249863644e-06
2 1.73767040223538e-06
3 1.65489782943951e-06
4 1.62000515047112e-06
5 1.60325535603079e-06
6 1.59140887490139e-06
7 1.57951745904938e-06
8 1.56983574584046e-06
};
\addplot [very thick, crimson2143940, mark=triangle*, mark size=5, mark options={solid,draw=white}]
table {%
1 1.67174763987532e-06
2 1.58122753646239e-06
3 1.52279605458716e-06
4 1.48431567481566e-06
5 1.4726347501437e-06
6 1.46166718195673e-06
7 1.4611167671319e-06
8 1.4608461356147e-06
};
\addplot [very thick, forestgreen4416044, mark=pentagon*, mark size=5, mark options={solid,draw=white}]
table {%
1 1.29855533259615e-06
2 1.29855405361923e-06
3 1.29855956743086e-06
4 1.29854697661358e-06
5 1.29855263253376e-06
6 1.29855817476709e-06
7 1.29856246644522e-06
8 1.29856201169787e-06
};
\addplot [very thick, steelblue31119180, mark=diamond*, mark size=5, mark options={solid,draw=white}]
table {%
1 1.60576516350375e-06
2 1.5344699590969e-06
3 1.50345218230541e-06
4 1.48669604982388e-06
5 1.47146081985738e-06
6 1.47769040381718e-06
7 1.47124487170913e-06
8 1.47071213518757e-06
};
\end{axis}
\end{tikzpicture}

==> figures/quantitative_results/sd/ml_loss/sd_ablation_context.tex <==
% This file was created with matplot2tikz v0.5.1.
\begin{tikzpicture}

\definecolor{crimson2143940}{RGB}{214,39,40}
\definecolor{darkgray}{RGB}{169,169,169}
\definecolor{darkorange25512714}{RGB}{255,127,14}
\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{forestgreen4416044}{RGB}{44,160,44}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{mediumpurple148103189}{RGB}{148,103,189}
\definecolor{steelblue31119180}{RGB}{31,119,180}

\begin{axis}[
    line width=0.8pt,             % Thicker axis outline
    axis line style={black},      % Solid black contrast
    log basis y={10},
    tick align=outside,
    % title={Sheet Deformation},
    xlabel={Context Size},
    xlabel style={font=\LARGE, color=black},
    % ylabel={Full Rollout MSE},
    ylabel style={font=\LARGE, color=black},
    tick label style={font=\large, color=black},
    xmajorgrids,
    xtick={1,2,3,4,5,6,7,8},           % Specify tick positions
    xticklabels={1,2,3,4,5,6,7,8},     % Specify tick labels
    xmajorticks=true,                  % Ensure ticks are enabled
    xtick pos=bottom,
    xmin=0.65, xmax=8.35,
    xtick style={color=black, line width=0.8pt},
    y grid style={lightgray!70},  % Darker grid lines
    ymajorgrids,
    % Kept your original y-range for Sheet Deformation
    ymin=3.02647033233786e-08, ymax=4.72304384868436e-05,
    ymode=log,
    ytick pos=left,
    ytick style={color=black, line width=0.8pt}
]
\path [draw=darkorange25512714, fill=darkorange25512714, opacity=0.2]
(axis cs:1,3.36614743901009e-05)
--(axis cs:1,2.65160761045991e-05)
--(axis cs:2,2.65160633716732e-05)
--(axis cs:3,2.65160815615673e-05)
--(axis cs:4,2.65160651906626e-05)
--(axis cs:5,2.65160842900514e-05)
--(axis cs:6,2.65160651906626e-05)
--(axis cs:7,2.65160615526838e-05)
--(axis cs:8,2.65160770140938e-05)
--(axis cs:8,3.36613748004311e-05)
--(axis cs:8,3.36613748004311e-05)
--(axis cs:7,3.3812106721598e-05)
--(axis cs:6,3.36614189109241e-05)
--(axis cs:5,3.36613820763887e-05)
--(axis cs:4,3.36651707698365e-05)
--(axis cs:3,3.3812126275734e-05)
--(axis cs:2,3.38121380991652e-05)
--(axis cs:1,3.36614743901009e-05)
--cycle;
\path [draw=mediumpurple148103189, fill=mediumpurple148103189, opacity=0.2]
(axis cs:1,5.88738842566272e-07)
--(axis cs:1,3.35676525331508e-07)
--(axis cs:2,1.85870671742805e-07)
--(axis cs:3,1.96925267204051e-07)
--(axis cs:4,1.95514850531708e-07)
--(axis cs:5,1.83973703826723e-07)
--(axis cs:6,1.84667015901141e-07)
--(axis cs:7,1.79375916786739e-07)
--(axis cs:8,1.75611702957212e-07)
--(axis cs:8,2.09818125540551e-07)
--(axis cs:8,2.09818125540551e-07)
--(axis cs:7,2.0945153522689e-07)
--(axis cs:6,2.10796272881453e-07)
--(axis cs:5,2.17816499059609e-07)
--(axis cs:4,2.29190582956562e-07)
--(axis cs:3,2.35318907471083e-07)
--(axis cs:2,2.2199241556109e-07)
--(axis cs:1,5.88738842566272e-07)
--cycle;
\path [draw=crimson2143940, fill=crimson2143940, opacity=0.2]
(axis cs:1,7.99657911443319e-07)
--(axis cs:1,4.95366769825978e-07)
--(axis cs:2,2.29571838872289e-07)
--(axis cs:3,2.2567823521058e-07)
--(axis cs:4,2.14074685089827e-07)
--(axis cs:5,2.05354318438822e-07)
--(axis cs:6,2.04547085047579e-07)
--(axis cs:7,2.02685072281383e-07)
--(axis cs:8,1.99070296247328e-07)
--(axis cs:8,2.60654125838755e-07)
--(axis cs:8,2.60654125838755e-07)
--(axis cs:7,2.5319228313947e-07)
--(axis cs:6,2.71147559516294e-07)
--(axis cs:5,2.72206335694136e-07)
--(axis cs:4,2.88310805807157e-07)
--(axis cs:3,2.89073540216123e-07)
--(axis cs:2,2.99039442097637e-07)
--(axis cs:1,7.99657911443319e-07)
--cycle;
\path [draw=forestgreen4416044, fill=forestgreen4416044, opacity=0.2]
(axis cs:1,4.80712571970798e-08)
--(axis cs:1,4.22752091111533e-08)
--(axis cs:2,4.22765928931312e-08)
--(axis cs:3,4.22761168294983e-08)
--(axis cs:4,4.22756762930021e-08)
--(axis cs:5,4.22754737883224e-08)
--(axis cs:6,4.22760813023615e-08)
--(axis cs:7,4.22762393981202e-08)
--(axis cs:8,4.22761363694235e-08)
--(axis cs:8,4.80717456952107e-08)
--(axis cs:8,4.80717456952107e-08)
--(axis cs:7,4.80716195738751e-08)
--(axis cs:6,4.80715307560331e-08)
--(axis cs:5,4.80718487239074e-08)
--(axis cs:4,4.80715627304562e-08)
--(axis cs:3,4.80713300277102e-08)
--(axis cs:2,4.80721435991427e-08)
--(axis cs:1,4.80712571970798e-08)
--cycle;
\path [draw=steelblue31119180, fill=steelblue31119180, opacity=0.2]
(axis cs:1,4.2036381842081e-07)
--(axis cs:1,1.9226405356676e-07)
--(axis cs:2,1.41688168753262e-07)
--(axis cs:3,1.40581622787295e-07)
--(axis cs:4,1.36576154829982e-07)
--(axis cs:5,1.32790113127612e-07)
--(axis cs:6,1.26062680294581e-07)
--(axis cs:7,1.23081605352127e-07)
--(axis cs:8,1.21796588814505e-07)
--(axis cs:8,1.69823117346368e-07)
--(axis cs:8,1.69823117346368e-07)
--(axis cs:7,1.70735770410602e-07)
--(axis cs:6,1.73041364348592e-07)
--(axis cs:5,1.76507832350126e-07)
--(axis cs:4,1.80823377604611e-07)
--(axis cs:3,1.84580066786566e-07)
--(axis cs:2,1.87385303718202e-07)
--(axis cs:1,4.2036381842081e-07)
--cycle;
\addplot [very thick, darkorange25512714, mark=*, mark size=5, mark options={solid,draw=white}]
table {%
1 2.90772063635814e-05
2 2.90771795334877e-05
3 2.90771822619718e-05
4 2.90771881736873e-05
5 2.90771822619718e-05
6 2.90771863546979e-05
7 2.90771654363198e-05
8 2.90771749860141e-05
};
\addplot [very thick, mediumpurple148103189, mark=square*, mark size=5, mark options={solid,draw=white}]
table {%
1 4.29895926856716e-07
2 2.01897488949498e-07
3 2.14529986664047e-07
4 2.10535318956317e-07
5 1.99196005468139e-07
6 1.95524226143107e-07
7 1.92447579649979e-07
8 1.91391933412888e-07
};
\addplot [very thick, crimson2143940, mark=triangle*, mark size=5, mark options={solid,draw=white}]
table {%
1 6.56739722160182e-07
2 2.60814303487678e-07
3 2.54909295449579e-07
4 2.49815663266872e-07
5 2.37835159566657e-07
6 2.35567323869645e-07
7 2.31347954127159e-07
8 2.28905921773048e-07
};
\addplot [very thick, forestgreen4416044, mark=pentagon*, mark size=5, mark options={solid,draw=white}]
table {%
1 4.51732331541166e-08
2 4.5174368246137e-08
3 4.51737234286043e-08
4 4.51736195117292e-08
5 4.51736612561149e-08
6 4.51738060291973e-08
7 4.51739294859976e-08
8 4.51739410323171e-08
};
\addplot [very thick, steelblue31119180, mark=diamond*, mark size=5, mark options={solid,draw=white}]
table {%
1 2.79103588241014e-07
2 1.63104733275077e-07
3 1.61079679372733e-07
4 1.58422608365072e-07
5 1.52170954947906e-07
6 1.48282151002377e-07
7 1.46461310635004e-07
8 1.45410574248217e-07
};
\end{axis}

\end{tikzpicture}


==> figures/quantitative_results/tikzcolors.tex <==
\definecolor{tabblue}{RGB}{31, 119, 180}
\definecolor{taborange}{RGB}{255, 127, 14}
\definecolor{tabgreen}{RGB}{44, 160, 44}
\definecolor{tabred}{RGB}{214, 39, 40}
\definecolor{tabpurple}{RGB}{148, 103, 189}
\definecolor{tabbrown}{RGB}{140, 86, 75}
\definecolor{tabpink}{RGB}{227, 119, 194}
\definecolor{tabgray}{RGB}{127, 127, 127}
\definecolor{tabolive}{RGB}{188, 189, 34}
\definecolor{tabcyan}{RGB}{23, 190, 207}
\definecolor{ForestGreen}{RGB}{34, 139, 34}

==> figures/quantitative_results_main_context.tex <==
\begin{figure}[t]
    \centering
    \makebox[\textwidth][c]{
    \input{figures/quantitative_results/legend}
    }
    \includegraphics[width=0.24\textwidth]{figures/quantitative_results/db/db_ml_loss.pdf}
    \includegraphics[width=0.24\textwidth]{figures/quantitative_results/db/db_mat_prop_loss.pdf}
    \includegraphics[width=0.24\textwidth]{figures/quantitative_results/sd/sd_ml_loss.pdf}
    \includegraphics[width=0.24\textwidth]{figures/quantitative_results/sd/sd_mat_prop_loss.pdf}
    \caption{
    Full simulation rollout and material property \gls{mse} across different encoder architectures as a function of the number of context sequences for (\textbf{left}) \texttt{Deforming Block} and (\textbf{right}) \texttt{Sheet Deformation}.
    \gls{peach} consistently performs similar to the mesh-based \gls{mango}, improving over other point cloud encoders and achieving near-Oracle performance on \texttt{Deforming Block}.
    }
    \label{fig:quantitative_comparison}
\end{figure}
